Declarative Policy Control for Data Spaces: A DSL-Based Approach for Manufacturing-X

The growing adoption of federated data spaces, such as in the GAIA-X and the International Data Spaces (IDS) initiative, promises secure and sovereign data sharing across organizational boundaries in Industry 4.0. In manufacturing ecosystems, this enables use cases, such as cross-factory process optimization, predictive maintenance, and supplier integration. Frameworks and standards, such as the Asset Administration Shell (AAS), Eclipse Dataspace Connector (EDC), ID-Link and Open Platform Communications Unified Architecture (OPC UA) provide a strong foundation to realize this ecosystem. However, a major open challenge is the practical description and enforcement of context-dependent data usage policies using these base technologies - especially by domain experts without software engineering backgrounds. Therefore, this article proposes a method for leveraging domain-specific languages (DSLs) to enable declarative, human-readable, and machine-executable policy definitions for sovereign data sharing via data space connectors. The DSL empowers domain experts to specify fine-grained data governance requirements - such as restricting access to data from specific production batches or enforcing automatic deletion after a defined retention period - without writing imperative code.

==> BiberConfig.tex <==
% ----------------------------------------
% BIBER Configuration
% ----------------------------------------
\usepackage[
  backend=biber, 
  style=authoryear-comp, 
  sortcites=false, 
  maxcitenames=2, 
  mincitenames=1, 
  maxbibnames=4, 
  uniquelist=false]{biblatex}

\DeclareFieldFormat{postnote}{\mknormrange{#1}}
\DeclareFieldFormat{volcitepages}{\mknormrange{#1}}
\DeclareFieldFormat{multipostnote}{\mknormrange{#1}}

\renewcommand*{\postnotedelim}{\addcolon}


\addbibresource{src/bib/andreaswortmann.bib}
\addbibresource{src/bib/references.bib}

\makeatletter
\def\nhblx@bibfile@name{\jobname -nhblx.bib}
\newwrite\nhblx@bibfile
\immediate\openout\nhblx@bibfile=\nhblx@bibfile@name

\immediate\write\nhblx@bibfile{%
  @comment{Auto-generated file}\blx@nl}

\newcounter{nhblx@name}
\setcounter{nhblx@name}{0}

\newcommand*{\nhblx@writenametobib}[1]{%
  \stepcounter{nhblx@name}%
  \edef\nhblx@tmp@nocite{%
    \noexpand\AfterPreamble{%
      \noexpand\setbox0\noexpand\vbox{%
        \noexpand\nhblx@getmethehash{nhblx@name@\the\value{nhblx@name}}}}%
  }%
  \nhblx@tmp@nocite
  \immediate\write\nhblx@bibfile{%
    @misc{nhblx@name@\the\value{nhblx@name}, author = {\unexpanded{#1}}, %
          options = {dataonly=true},}%
  }%
}

\AtEndDocument{%
  \closeout\nhblx@bibfile}

\addbibresource{\nhblx@bibfile@name}

\newcommand*{\nhblx@boldhashes}{}
\DeclareNameFormat{nhblx@hashextract}{%
  \xifinlist{\thefield{hash}}{\nhblx@boldhashes}
    {}
    {\listxadd{\nhblx@boldhashes}{\thefield{hash}}}}

\DeclareCiteCommand{\nhblx@getmethehash}
  {}
  {\printnames[nhblx@hashextract][1-999]{author}}
  {}
  {}

\newcommand*{\addboldnames}{\forcsvlist\nhblx@writenametobib}
\newcommand*{\resetboldnames}{\def\nhblx@boldhashes{}}

\newcommand*{\mkboldifhashinlist}[1]{%
  \xifinlist{\thefield{hash}}{\nhblx@boldhashes}
    {\mkbibbold{#1}}
    {#1}}
\makeatother

\DeclareNameWrapperFormat{boldifhashinlist}{%
  \renewcommand*{\mkbibcompletename}{\mkboldifhashinlist}%
  #1}

\DeclareNameWrapperAlias{sortname}{default}
\DeclareNameWrapperAlias{default}{boldifhashinlist}

%\addboldnames{Alexander Verl}
%\addboldnames{Andreas Wortmann}


% \DeclareBibliographyDriver{std}{%
%   \usebibmacro{bibindex}%
%   \usebibmacro{begentry}%
%   \usebibmacro{author/editor+others/translator+others}%
%   \setunit{\labelnamepunct}\newblock
%   \usebibmacro{title}%
%   \newunit\newblock
%   \usebibmacro{date}%
%   \newunit\newblock
%   \usebibmacro{finentry}}
  
  
% \DeclareBibliographyAlias{article}{std}
% \DeclareBibliographyAlias{book}{std}
% \DeclareBibliographyAlias{booklet}{std}
% \DeclareBibliographyAlias{collection}{std}
% \DeclareBibliographyAlias{inbook}{std}
% \DeclareBibliographyAlias{incollection}{std}
% \DeclareBibliographyAlias{inproceedings}{std}
% \DeclareBibliographyAlias{manual}{std}
% \DeclareBibliographyAlias{misc}{std}
% \DeclareBibliographyAlias{online}{std}
% \DeclareBibliographyAlias{patent}{std}
% \DeclareBibliographyAlias{periodical}{std}
% \DeclareBibliographyAlias{proceedings}{std}
% \DeclareBibliographyAlias{report}{std}
% \DeclareBibliographyAlias{thesis}{std}
% \DeclareBibliographyAlias{unpublished}{std}
% \DeclareBibliographyAlias{*}{std}

% Content Tailoring
%
% tailor content of bibliography
\AtEveryBibitem{
   \clearfield{month}
   \clearfield{series}
   \clearfield{venue}
   \clearname{editor}
   \clearlist{publisher}
   \clearlist{location} % alias to field 'address'
   \clearfield{doi}
   \clearfield{url}
   \clearfield{venue}
   \clearfield{issn}
   \clearfield{isbn}
   \clearfield{urldate}
   \clearfield{eventdate}
   \clearfield{pages}
   %\clearfield{booktitle}
   %\clearfield{journaltitle}
   %\clearfield{number}
   %\clearfield{volume}
}
